View-Based Owicki-Gries Reasoning for Persistent x86-TSO (Extended Version)

The rise of persistent memory is disrupting computing to its core. Our work aims to help programmers navigate this brave new world by providing a program logic for reasoning about x86 code that uses low-level operations such as memory accesses and fences, as well as persistency primitives such as flushes. Our logic, Pierogi, benefits from a simple underlying operational semantics based on views, is able to handle optimised flush operations, and is mechanised in the Isabelle/HOL proof assistant. We detail the proof rules of Pierogi and prove them sound. We also show how Pierogi can be used to reason about a range of challenging single- and multi-threaded persistent programs.

==> mechanisation.tex <==
\section{Mechanisation}
\label{sec:mechanisation}


% \BD{WRT to other mechanisations, the focus of our work has been the
% Isabelle/HOL verification tool, which provides a reusable framework}

% % \BD{Breakdown number of lines (DONE) + person hours (DONE) + compile time }


% \OL{one thing that is different here than in other formalization papers is that 
% we don't really formalize the soundness meta-theory. Instead we formalize the reasoning about examples}
% % \BD{Do we want to say this? Or say that the metatheory is standard?}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

